Gradient Approximation and Multi-Variable Derivative-Free Optimization based on Non-Commutative Maps

In this work, multi-variable derivative-free optimization algorithms for unconstrained optimization problems are developed. A novel procedure for approximating the gradient of multi-variable objective functions based on non-commutative maps is introduced. The procedure is based on the construction of an exploration sequence to specify where the objective function is evaluated and the definition of so-called gradient generating functions which are composed with the objective function such that the procedure mimics a gradient descent algorithm. Various theoretical properties of the proposed class of algorithms are investigated and numerical examples are presented.

==> myStandardPreamble_arXiv.tex <==
% change @-symbol interpretation for using macros
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% =============================
% ===         M I S C      ====
% =============================

% extended TeX
\@ifpackageloaded{etex}{}{\RequirePackage{etex}}

% keeps relative paths when including different .tex-files
% use \subimport*{subdirectory}{tex-File} to input tex-Files
\@ifpackageloaded{import}{}{\usepackage{import}}

% nice tables
\@ifpackageloaded{booktabs}{}{\usepackage{booktabs}}

% microtype for better spacing of letters
%\@ifpackageloaded{microtype}{}{\usepackage{microtype}}

% calculations also in tex-Code
\@ifpackageloaded{calc}{}{\usepackage{calc}}

% if conditions
\@ifpackageloaded{ifthen}{}{\usepackage{ifthen}}


% =============================
% ===    G R A P H I C S    ===
% =============================
\@ifpackageloaded{graphicx}{}{\usepackage{graphicx}}
\@ifpackageloaded{xcolor}{}{\usepackage{xcolor}}


% =============================
% ===         T I K Z      ====
% =============================
\@ifpackageloaded{tikz}{
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
     }{
     \usepackage{tikz}
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
}
\@ifpackageloaded{pgfplots}{
     }{
     \usepackage{pgfplots}
     }
% SOME TIKZ STYLE DEFINITIONS
\tikzstyle{boxstyle}=[draw=black,inner sep=7pt]      % style for boxes in blockdiagrams
\tikzstyle{arrowstyle}=[]                            % style for arrows in blockdiagrams



% =============================
% ===         M A T H      ====
% =============================
\@ifpackageloaded{amsmath}{}{\usepackage{amsmath}}
\@ifpackageloaded{amsfonts}{}{\usepackage{amsfonts}}
\@ifpackageloaded{amssymb}{}{\usepackage{amssymb}}
\let\theoremstyle\relax
\@ifpackageloaded{amsthm}{}{\usepackage{amsthm}}
\@ifpackageloaded{yhmath}{}{\usepackage{yhmath}}
\@ifpackageloaded{mathdots}{}{\usepackage{mathdots}}


% =============================
% ===    H Y P E R R E F    ===
% =============================

% some color definitions
\colorlet{lcolor}{green!45!black}
\colorlet{ucolor}{magenta!40!black}
\colorlet{ccolor}{green!40!black}

% hyperref for internal links
\usepackage[colorlinks=true,%
            linkcolor=lcolor,%
            urlcolor=lcolor,%
            citecolor=lcolor]{hyperref}

% cleverref for automatically labeling of references
\usepackage[nameinlink,capitalise]{cleveref}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% rechange @-symbol interpretation
\makeatother


==> subfiles/simulations.tex <==
In this section we study our discrete-time derivative-free optimization algorithms \eqref{eq:algos} in various simulation examples and provide some tuning rules. To this end, we consider the cost function $J(x) = (x - 2)^2 + 6$. If not otherwise specified we use the vector fields \eqref{eq:vec_sincos} and initialize the algorithms with $x_0=x(0) = 0.5$. For the sake of convenience we define this setup as $\mathcal{P}:=\left(J,x_0,\fJ_1,\fJ_2\right)$. Note that the results obtained with such a quadratic cost function also provide insight into the results that would be obtained with an arbitrary function of class $C^2$ near a minimum
with positive definite Hessian.
%
We start by analyzing \eqref{eq:algos}, applied to the basic setup $\mathcal{P}$, which is depicted for (a large) step size $h=0.5$ in~\Cref{fig:sim_dES}, where the switching of the vector fields $\fJ_1,\fJ_2$ is highlighted. 
\pgfplotsset{minor grid style={dotted}}
As it can be observed, the trajectories of $x_k$ are converging into a neighborhood of $x^*$, which is of order $\mathcal{O}(\sqrth)$ (see proof of~\Cref{thm:conv}).
To eliminate the steady-state oscillatory behavior, we propose the filter $y_{k+1} = y_k + \frac{1}{4n}\sum_{i=k-4n}^{k-1} x_{i+1}-x_{i}$
where $y_0= x_0$ and $x_l = x_0,\ l<0$, which shows a good asymptotic convergence behavior of the algorithms \eqref{eq:algos} to the extremum $x^*$ as illustrated in~\Cref{fig:sim_dES}. 
\begin{figure}[t]
	\centering
	\setlength\figureheight{3.9cm}
	\setlength\figurewidth{7.5cm}
	{\small \input{Fig/dES.tikz}}
	\caption[]{Convergence of $x_k$ in \eqref{eq:algos}  for setup $\mathcal{P}$ with $h=0.5$ to a neighborhood of $x^*=2$. The flow maps as in \eqref{eq:algo_flow} for $M=E$ are highlighted with $E_{\fJ_1}^{\sqrth}$ ({\color{red}$\boldmin$}), $E_{\fJ_2}^{\sqrth}$ ({\color{green}$\boldmin$}),  $E_{-\fJ_1}^{\sqrth}$ ({\color{blue}$\boldmin$}), $E_{-\fJ_2}^{\sqrth}$ ({\color{orange}$\boldmin$}) and the same color scheme (dotted) for \eqref{eq:algo_flow}, $M=H$. This is compared with the trajectory resulting from a gradient descent algorithm with the exact gradient ($\thinmin$). By filtering $x_k$, a good asymptotic convergence behavior of $y_k$ to $x^*$ can be observed ({\color{gray}$\thinmins\,\thinmins$}).}
	\label{fig:sim_dES}
\end{figure}
Obviously, $y_k$ is a windowed filter with length $4n$, which is not fed back into the algorithm.
This behavior can also be observed in a multidimensional optimization problem as depicted in~\Cref{fig:sim_dES2D}.  
\begin{figure}[t]
	\centering
	\setlength\figureheight{5.5cm}
	\setlength\figurewidth{7cm}
	{\small \input{Fig/dES2D.tikz}}
	\caption[]{A two-dimensional optimization problem with $J(x)=(x^1-2)^2+(x^2-2)^2+6$. Trajectories $x_k$ ({\color{orange}$\boldmin$}) of \eqref{eq:algo_euler} and $y_k$ ({\color{green}$\boldmin$}) converge to the extremum $x^*=[2,2]$ ($\red{\bullet}$) initialized with $x_0=y_0=[0.5,0.5]$ ($\bullet$).}
	\label{fig:sim_dES2D}
\end{figure}

As known from continuous-time methods, see for example \cite{durr2013lie}, increasing the (switching) frequency, and hence reducing the step size $h$, leads to a convergence into a smaller neighborhood around $x^*$ as depicted for different $h$'s in~\Cref{fig:sim_dES_diff_h}.
Clearly, for decreasing the step size, more iterations are needed, hence more function evaluations.
\begin{figure}[t]
	\centering
	\setlength\figureheight{3.9cm}
	\setlength\figurewidth{7.5cm}
	{\small \input{Fig/dES_diff_h.tikz}}
	\caption[]{Choosing smaller step sizes for algorithm \eqref{eq:algo_euler} or \eqref{eq:algo} yield to a smaller neighborhood of convergence. Trajectories of $x_k$ for setup $\mathcal{P}$ with step sizes $h=0.5$ ({\color{green}$\boldmin$}), $h=0.1$ ({\color{blue}$\boldmin$}), $h=0.01$ ({\color{orange}$\boldmin$}), $h=0.001$ ({\color{brown}$\boldmin$}).}
	\label{fig:sim_dES_diff_h}
\end{figure}

As mentioned in~\Cref{sec:intro}, an advantage of the proposed class of algorithms is robustness with respect to noisy objective functions.
Therefore, consider the setup $\mathcal{P}$, but with a noisy cost function $\bar{J}:\mathbb{R}\rightarrow \mathbb{R}$ such that
\begin{align}
	\bar{J}(x_k) \sim \mathcal{N}(J(x_k),0.04),
\end{align} 
where $\mathcal{N}(J(x_k),0.04)$ is a normal distribution with mean $J(x_k)$ and standard derivation $\sqrt{0.04}=0.2$. In~\Cref{fig:sim_dES_noise}, algorithm \eqref{eq:algo} is compared with the well known difference quotient method to approximate the gradient $D(J(\bar{x})):= h^{-1}(J(\bar{x}_k)-J(\bar{x}_k+h))$ used in a gradient descent algorithm $\bar{x}_{k+1}=\bar{x}_k-hD(J(\bar{x}))$ with step size $h = 0.01$ and initial condition $\bar{x}_0 = x_0$. 
\begin{figure}[t]
	\centering
	\setlength\figureheight{3.9cm}
	\setlength\figurewidth{7.5cm}
	{\small \input{Fig/dES_noise.tikz}}
	\caption[]{Study of noisy objective function: trajectory $x_k$ of algorithm \eqref{eq:algo} ({\color{green}$\boldmin$}), trajectory $\bar{x}_k$ of gradient descent with gradient approximation via difference quotient ({\color{orange}$\boldmin$}), trajectory of gradient descent with exact gradient ({\color{black}$\boldmin$}).}
	\label{fig:sim_dES_noise}
\end{figure}
Apparently, approximating the gradient via the difference quotient method is much more sensitive regarding noisy objectives as algorithms \eqref{eq:algos}. This is reasoned by the averaging behavior of the proposed algorithms, implied by utilizing non-commutative maps. 

Concluding, we illustrated both algorithms \eqref{eq:algos} on simple examples and we introduced a filtering method. Secondly, we showed the impact of decreasing $h$ and the performance under noisy measurements. Regarding the convergence behavior, algorithm \eqref{eq:algo_euler} and \eqref{eq:algo} show similar convergence behavior for the considered vector fields \eqref{eq:vec_sincos} and switching function \eqref{eq:seq_switch_seq_n}. Nevertheless, algorithm \eqref{eq:algo} needs two times more function evaluations than \eqref{eq:algo_euler}. 
